Database Research needs an Abstract Relational Query Language

For decades, SQL has been the default language for composing queries, but it is increasingly used as an artifact to be read and verified rather than authored. With Large Language Models (LLMs), queries are increasingly machine-generated, while humans read, validate, and debug them. This shift turns relational query languages into interfaces for back-and-forth communication about intent, which will lead to a rethinking of relational language design, and more broadly, relational interface design. We argue that this rethinking needs support from an Abstract Relational Query Language (ARQL): a semantics-first reference metalanguage that separates query intent from user-facing syntax and makes underlying relational patterns explicit and comparable across user-facing languages. An ARQL separates a query into (i) a relational core (the compositional structure that determines intent), (ii) modalities (alternative representations of that core tailored to different audiences), and (iii) conventions (orthogonal environment-level semantic parameters under which the core is interpreted, e.g., set vs. bag semantics, or treatment of null values). Usability for humans or machines then depends less on choosing a particular language and more on choosing an appropriate modality. Comparing languages becomes a question of which relational patterns they support and what conventions they choose. We introduce Abstract Relational Calculus (ARC), a strict generalization of Tuple Relational Calculus (TRC), as a concrete instance of ARQL. ARC comes in three modalities: (i) a comprehension-style textual notation, (ii) an Abstract Language Tree (ALT) for machine reasoning about meaning, and (iii) a diagrammatic hierarchical graph (higraph) representation for humans. ARC provides the missing vocabulary and acts as a Rosetta Stone for relational querying.

==> datalabmacros.tex <==

\usepackage{anyfontsize}	%
\usepackage[T1]{fontenc} %


\setlength{\mathindent}{0pt}  %


\usepackage{amsthm}
\usepackage{graphicx} %
\usepackage{subcaption}
\usepackage{placeins}
\usepackage{float}
\usepackage{afterpage}
\usepackage{url}
\usepackage{enumitem} %
\newcommand{\bmmax}{3}	%
\usepackage{bm} %
\usepackage{upgreek} %
\usepackage{soul} %
\usepackage{bbding} %
\usepackage{pifont} %
\usepackage{listings} %

\usepackage{tabularx} %
\usepackage{booktabs} %
\usepackage{multirow}
\usepackage{hhline} %
\usepackage{diagbox}

\usepackage{booktabs}  %

\usepackage{tikz} %
\usetikzlibrary{positioning}

\usepackage{wasysym}	%



\RequirePackage{etoolbox}	%
\newcommand{\iflabelexists}[3]{\ifcsundef{r@#1}{#3}{#2}}


\usepackage{wrapfig}
\usepackage{cutwin}






\usepackage{adjustbox}
\def\eox{\unskip\kern 10pt{\unitlength1pt\linethickness{.4pt}$\diamondsuit${}}} %

\usepackage{easybmat} %


\usepackage{rotating}		%






\usepackage{svg}


\usepackage{pgfplotstable} %


\sloppy %





\let\subcaption\relax
\let\subfloat\relax
\usepackage{subcaption}		%
\captionsetup[figure]{font=small}		%
\captionsetup[table]{font+=small}		%
\captionsetup[subfigure]{font+=small}	%
\captionsetup[figure]{aboveskip=3pt}







\usepackage[ruled,noend,linesnumbered]{algorithm2e} %

\DontPrintSemicolon     %
\SetNlSty{}{}{}                %
\SetAlgoInsideSkip{smallskip}   %
\SetAlCapSkip{1.5mm}             %
\setlength{\algomargin}{1.5mm}    %
\SetInd{1.5mm}{1.5mm}             %

\SetAlFnt{\small}			%
\SetAlCapFnt{\small}		%
\SetAlCapNameFnt{\small}





\newtheorem{hypothesis}{Hypothesis}






\newcommand{\todo}[1]{{\color{red}[\textbf{TODO}:{#1}]}} %
\newcommand{\wolf}[1]{{{\color{red}{[\textbf{wg}: #1]}}}} %
\newcommand{\diandre}[1]{{{\color{blue}{[\textbf{ds}: #1]}}}}
\newcommand{\cody}[1]{{{\color{orange}{[\textbf{cd}: #1]}}}} %
\newcommand{\cd}[2]{{{\color{orange}{[\textbf{cd (#1)}: #2]}}}} %
\newcommand{\deprecate}[1]{{{\color{gray}{#1}}}} %
\newcommand{\out}[1]{{\color{gray}\textbf{OUT}: #1}}


\newcommand{\later}[1]{{\color{blue}\textbf{LATER}: #1}}
\newcommand{\laterr}[1]{}

\newcommand{\revision}[1]{{\color{blue}{#1}}}



\newcommand{\hide}[1]{} 		%




\newcommand{\addformat}[1]{\textcolor{blue}{#1}} 
\newcommand{\removeformat}[1]{\textcolor{red}{#1}}



\newcommand{\mkclean}{
    \renewcommand{\out}[1]{\hide}
    \renewcommand{\todo}{\hide}
    \renewcommand{\deprecate}{\hide}
    \renewcommand{\wolf}[1]{\hide}
    \renewcommand{\cody}[1]{\hide}	
    \renewcommand{\cd}[2]{\hide}	
}
















\usepackage[capitalise,nameinlink]{cleveref} %

\crefname{algocf}{Alg.}{Algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefalias{AlgoLine}{line}%
\crefname{property}{Property}{Properties}

\crefformat{equation}{(#2#1#3)}						%
\crefrangeformat{equation}{(#3#1#4) to~(#5#2#6)}
\crefmultiformat{equation}{(#2#1#3)}%
{ and~(#2#1#3)}{, (#2#1#3)}{ and~(#2#1#3)}






\AtEndPreamble{%
    \hypersetup{colorlinks,
      linkcolor=ACMDarkBlue,		%
      citecolor=blue,
      urlcolor=ACMDarkBlue,
      filecolor=ACMDarkBlue,
      pdfcreator = {},
      }}










	
	\usepackage[normalem]{ulem} %
	\newcommand\highl{\bgroup\markoverwith
	  {\textcolor{yellow}{\rule[-.5ex]{2pt}{2.5ex}}}\ULon}





\usepackage{marginnote}
\newcommand{\rebuttal}[2]{\marginnote{\textbf{\textcolor{blue}{#1}}}{\color{blue}#2}}
\newcommand{\new}[1]{{\color{blue}{#1}}}








\usepackage{tcolorbox}		%
\tcbuselibrary{breakable,skins}		%


\tcbset{examplestyle/.style={
	enhanced jigsaw,	%
	colback=gray!10,	%
	colframe=gray!20,	%
	arc=0mm,			%
	boxrule=1pt,		%
	left=1mm,
	right=1mm,
	left skip=0mm,  %
	right skip=0mm, %
	top=1mm,		%
	bottom=1mm,		%
	breakable,		%
	parbox = false,		%
	before={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},
	after={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},				
	boxsep = 0mm,					%
	topsep at break=0pt,			%
	bottomsep at break=0pt,			%
	pad at break=0mm,
	pad before break=0mm,		
	pad after break=1mm,		
	bottomrule at break=0mm,
	toprule at break=0mm,		
	}}

\tcolorboxenvironment{example}{examplestyle}



\newtheoremstyle{abcd}%
  {}%
  {}%
  {\upshape}%
  {}%
  {\itshape}%
  {.}%
  {.5em}%
  {}%

\theoremstyle{abcd}
\newtheorem{example}{Example}




\tcbset{theoremstyle/.style={
		enhanced jigsaw,	%
		colback=white,	%
		colframe=black,	%
		arc=0mm,			%
		boxrule=1pt,		%
		left=1mm,
		right=1mm,
		left skip=0mm,  %
		right skip=0mm, %
		top=1mm,		%
		bottom=1mm,		%
		breakable,		%
		parbox = false,		%
		before={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},
		after={\par\pagebreak[0]\vspace{1mm}\parindent=0pt},				
		boxsep = 0mm,					%
		topsep at break=0pt,			%
		bottomsep at break=0pt,			%
		pad at break=0mm,
		pad before break=0mm,		
		pad after break=1mm,		
		bottomrule at break=0mm,
		toprule at break=0mm,		
		}}

\tcolorboxenvironment{theorem}{theoremstyle}
\tcolorboxenvironment{corollary}{theoremstyle}



\newtheoremstyle{abcd}%
  {}%
  {}%
  {\itshape}%
  {}%
  {\scshape}%
  {.}%
  {.5em}	%
  {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}%

\theoremstyle{abcd}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{corollary}













\tcbset{qrboxstyle/.style={
		enhanced jigsaw,	%
		colback=gray!20,
		colframe=gray!40,
		arc=0mm,
		boxrule=1pt,		%
		left=1pt,
		right=1pt,
		topsep at break=1mm,			%
		top=1pt,		%
		bottom=0mm,		%
		breakable,		%
		parbox = false		%
		}}


\newcommand{\resultbox}[1]{
\begin{tcolorbox}[
	enhanced jigsaw,		%
	colback=red!5,
	colframe=red!75!black,	
	arc=0mm,
	left skip=0mm,
	right skip=0mm,	
	left=0mm,
	topsep at break=1mm,			%
	right=0mm,
	top=0mm,
	bottom=0mm,		%
	breakable,		%
	parbox = false		%
]
\emph{#1}
\end{tcolorbox}
}


\newcounter{resultboxenv}

\newsavebox{\coloredbgbox}
\newenvironment{resultboxenv}{
	\begin{lrbox}{\coloredbgbox}
		\begin{minipage}{\dimexpr1\linewidth-2\fboxsep-2\fboxrule\relax}
			\refstepcounter{resultboxenv}
			\emph{Result \theresultboxenv.}
			\itshape
		}
  		{
		\end{minipage}
	\end{lrbox}
	\begin{center}
		\fcolorbox{black}{black!05}{\usebox{\coloredbgbox}}
	\end{center}
}



\newtheorem{resultW}{Result}

\renewenvironment{resultW}[1][]
{%
\par\noindent
  {\textbf{Result \arabic{resultW}#1.}
  \stepcounter{resultW}}%
  \begin{itshape}%
}%
{\end{itshape}
}
\setcounter{resultW}{1}

\newtheorem{resultE}{Pilot Result}

\renewenvironment{resultE}[1][]
{%
\par\noindent
  {\textbf{Pilot Result \arabic{resultE}#1.}
  \stepcounter{resultE}}%
  \begin{itshape}%
}%
{\end{itshape}
}
\setcounter{resultE}{1}






\renewcommand\dbltopfraction{1} %
\renewcommand\topfraction{1} 	%
\setcounter{dbltopnumber}{8}	%
\setcounter{topnumber}{8}		%






\usepackage{adjustbox}
\def\eox{\unskip\kern 10pt{\unitlength1pt\linethickness{.4pt}$\diamondsuit${}}}   




	





\makeatletter
\DeclareRobustCommand*\uell{\mathpalette\@uell\relax}
\newcommand*\@uell[2]{
  \setbox0=\hbox{$#1\ell$}
  \setbox1=\hbox{\rotatebox{10}{$#1\ell$}}
  \dimen0=\wd0 \advance\dimen0 by -\wd1 \divide\dimen0 by 2
  \mathord{\lower 0.1ex \hbox{\kern\dimen0\unhbox1\kern\dimen0}}
}
\makeatother





\newcommand{\smallsection}[1]{\vspace{5mm}\noindent\textbf{#1.}} %
\newcommand{\introparagraph}[1]{\textbf{#1.}} %

\newcommand{\ourmethod}{\textsc{QueryVis} \color{red}{TEST TEST TEST TEST !!!!}\xspace}
\renewcommand{\epsilon}{\varepsilon} %
\newcommand{\set}[1]{\{#1\}}                    %
\newcommand{\setof}[2]{\{{#1}\mid{#2}\}}        %

\newcommand{\define}{\stackrel{\textup{\tiny def}}{=}}

\newcommand{\datarule}{{\,:\!\!-\,}} %
\renewcommand{\vec}[1]{\boldsymbol{\mathbf{#1}}}
\newcommand{\transpose}{\intercal}	%

\newcommand{\N}{\mathbb{N}} %
\newcommand{\R}{{\mathbb{R}}} %
\newcommand{\bigO}{{\mathcal{O}}} %
\renewcommand{\O}{{\mathcal{O}}} %
\renewcommand{\P}{{\mathbb{P}}} %
\newcommand{\PP}[1]{\mathbb{P} [ #1 ]} %
\newcommand{\sql}[1]{\textrm{{#1}}}
\newcommand{\datastyle}[1]{\texttt{#1}}






\usepackage{caption}
    
    

\usepackage{bm}

\newcommand{\qv}{QV\xspace}


\newcommand{\formattedurl}[2]{\href{#1}{\small\texttt{#2}}\xspace}







\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}
\definecolor{myred}{rgb}{1,0,0}
\definecolor{mylightblue}{rgb}{0.953, 0.957, 0.980} 	%
\definecolor{mylightblueborder}{rgb}{0.567, 0.627, 0.757} 	%
\definecolor{mylightyellow}{rgb}{0.988, 0.957, 0.863} 	%



\lstset{ 
  backgroundcolor=\color{mylightyellow},   %
  rulecolor=\color{mylightblueborder},         %
  basicstyle=\footnotesize\ttfamily\linespread{0.75},        %
  breakatwhitespace=false,         %
  breaklines=true,                 %
  captionpos=b,                    %
  commentstyle=\color{mygreen},    %
  deletekeywords={...},            %
  escapeinside={\%*}{*)},          %
  extendedchars=true,              %
  frame=single,	                   %
  keepspaces=true,                 %
  numbers=none,                    %
  numbersep=5pt,                   %
  numberstyle=\tiny\color{mygray}, %
  showspaces=false,                %
  showstringspaces=false,          %
  showtabs=false,                  %
  stepnumber=1,                    %
  stringstyle=\color{mymauve},     %
  tabsize=2,	                   %
  title=\lstname,                  %
  classoffset=0,
  morekeywords={SELECT, DISTINCT, FROM, WHERE, AND, OR, AS, ON, HAVING, 
  	SUM, AVG, COUNT,
  	select, distinct, from, where, and, as, on, having,
	sum, avg, count, exists, or, join, lateral, JOIN, LATERAL,
	GROUP, BY, group, by, into, true, left, not, in, is, null},            %
  keywordstyle=\color{blue},       %
  classoffset=1,%
  morekeywords={SELECT},
  keywordstyle=\color{blue},
  classoffset=2,%
  morekeywords={any, all, OR, UNION, IN, ANY, ALL, NOT, 	EXISTS, LEFT,  IS, NULL},
  keywordstyle=\color{myred},
  classoffset=3,%
  morekeywords={test},
  keywordstyle=\color{mymauve},
  classoffset=4,%
  morekeywords={query, block1, block2, block3, block4, qb1, qb2, qb3, qb4, subquery2},
  keywordstyle=\color{gray},  
  classoffset=0,%
}








\RequirePackage{scalerel}
\RequirePackage{tikz}
\usetikzlibrary{svg.path}

\definecolor{orcidlogocol}{HTML}{A6CE39}
\tikzset{
  orcidlogo/.pic={
    \fill[orcidlogocol] svg{M256,128c0,70.7-57.3,128-128,128C57.3,256,0,198.7,0,128C0,57.3,57.3,0,128,0C198.7,0,256,57.3,256,128z};
    \fill[white] svg{M86.3,186.2H70.9V79.1h15.4v48.4V186.2z}
                 svg{M108.9,79.1h41.6c39.6,0,57,28.3,57,53.6c0,27.5-21.5,53.6-56.8,53.6h-41.8V79.1z M124.3,172.4h24.5c34.9,0,42.9-26.5,42.9-39.7c0-21.5-13.7-39.7-43.7-39.7h-23.7V172.4z}
                 svg{M88.7,56.8c0,5.5-4.5,10.1-10.1,10.1c-5.6,0-10.1-4.6-10.1-10.1c0-5.6,4.5-10.1,10.1-10.1C84.2,46.7,88.7,51.3,88.7,56.8z};
  }
}

\RequirePackage{etoolbox}
\DeclareRobustCommand\orcidicon[1]{\href{https://orcid.org/#1}{\mbox{\scalerel*{
\begin{tikzpicture}[yscale=-1, transform shape]
    \pic{orcidlogo};
\end{tikzpicture}
}{|}}}}
 




\newcommand{\equal}{\!=\!}

\let\oldin\in
\renewcommand{\in}{\!\oldin\!}
\renewcommand{\L}{\mathcal{L}}

\newcommand{\rep}{\textrm{rep}}
\newcommand{\ex}{\textrm{exp}}

\newcommand{\RA}{\textsf{RA}}
\newcommand{\NDRA}{\RA^{*}}
\newcommand{\NDRAPlain}{\RA*}
\newcommand{\NDRAA}{\RA^{*\antijoin}}

\newcommand{\Datalog}{\textsf{Datalog}}
\newcommand{\DatalogN}{\Datalog^{\neg}}
\newcommand{\DatalogND}{\Datalog^{*}}

\newcommand{\FOL}{\textsf{FOL}}
\newcommand{\DRC}{\textsf{DRC}}
\newcommand{\TRC}{\textsf{TRC}}
\newcommand{\ARC}{\textsf{ARC}}
\newcommand{\GTRC}{\textsf{G-TRC}}
\newcommand{\RC}{\textsf{RC}}
\newcommand{\NDTRC}{\TRC^{*}}
\newcommand{\NDTRCPlain}{\TRC*}

\newcommand{\SQL}{\textsf{SQL}\xspace}
\newcommand{\NDSQL}{\textsf{SQL}^{*}}


\newcommand{\NRD}{\textsf{RD}^{*}}
\newcommand{\RD}{\textsf{RD}}

\newcommand{\QBE}{\textsf{QBE}}


\newcommand{\queryviz}{\textsf{QueryVis}}
\newcommand{\demoname}{\textsf{PatternVis}}


 


\newcommand{\diagram}{\textsf{Relational Diagram}}
\newcommand{\diagrams}{\textsf{Relational Diagrams}}

\newcommand{\diagramNDnomath}{\texorpdfstring{\textsf{Relational Diagram}$^{*}$}{\textsf{Relational Diagram*}}}

\newcommand{\diagramsNDnomath}{\texorpdfstring{\textsf{Relational Diagrams}$^{*}$}{\textsf{Relational Diagrams*}}}
\newcommand{\diagramsND}{{\textsf{Relational Diagrams}^{*}}}	%














\definecolor{carfigORcolor}{HTML}{e77a30}

\newcommand{\h}[1]{\textcolor{red}{#1}} 	%
\newcommand{\hb}[1]{\textcolor{carfigORcolor}{#1}} 	%

\newcommand{\var}{\mathit{var}} 		
\newcommand{\const}{\mathit{const}} 	

\newcommand{\symb}{\bullet\;} 	

\newcommand{\antijoin}{\triangleright}

\newcommand{\tablesandattributes}{\textbf{Tables \& attributes}\xspace}
\newcommand{\constqualifications}{\textbf{Selection predicates}\xspace}
\newcommand{\joinattr}{\textbf{Join predicates}\xspace}
\newcommand{\quantifiers}{\textbf{Quantifiers}\xspace}
\newcommand{\nestingorder}{\textbf{Nesting order}\xspace}

\newcommand{\ittablesandattributes}{\emph{Tables \& attributes}\xspace}
\newcommand{\itconstqualifications}{\emph{Selection predicates}\xspace}
\newcommand{\itjoinattr}{\emph{Join predicates}\xspace}
\newcommand{\itquantifiers}{\emph{Quantifiers}\xspace}
\newcommand{\itnestingorder}{\emph{Nesting order}\xspace}

\definecolor{selPredicateColor}{HTML}{FFFFFF} 
\definecolor{selectBoxColor}{HTML}{BFBFBF}

\setlength{\fboxsep}{2pt}
\newcommand{\selPredicateBox}[1]{\fcolorbox{black}{selPredicateColor}{\textcolor{black}{#1}}}
\newcommand{\tableBox}[1]{\fcolorbox{black}{black}{\textcolor{white}{#1}}}
\newcommand{\attributeBox}[1]{\fcolorbox{black}{white}{\textcolor{black}{#1}}}
\newcommand{\selectBox}{\fcolorbox{black}{selectBoxColor}{\textcolor{white}{Q}}}


\newcommand{\E}{\mathcal{E}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\schema}{\textsf{schema}}

\newcommand{\countagg}{\textsf{count}}




\newlist{pfparts}{description}{1}
\setlist[pfparts,1]{%
    font=\normalfont\textsf,
    itemindent=2pt,
    wide,
    itemsep=.5em,topsep=.5em,
    labelsep=0.75ex
}
\makeatletter
\def\namedlabel#1#2{\begingroup
    #2%
    \def\@currentlabel{#2}%
    \phantomsection\label{#1}\endgroup
}
\makeatother





\newcommand{\osfpreprintplain}{osf.io/btszh}
\newcommand{\osfsupplementplain}{osf.io/mycr2}
\newcommand{\osfpreregplain}{osf.io/mycr2}

\newcommand{\osfpreprint}{\formattedurl{https://\osfpreprintplain}{\osfpreprintplain}}
\newcommand{\osfpreprintlong}{\formattedurl{https://\osfpreprintplain}{https://\osfpreprintplain}}

\newcommand{\osfsupplement}{\formattedurl{https://\osfsupplementplain}{\osfsupplementplain}}
\newcommand{\osfsupplementlong}{\formattedurl{https://\osfsupplementplain}{https://\osfsupplementplain}}

\newcommand{\osfprereg}{\formattedurl{https://\osfpreregplain}{\osfpreregplain}}


\usepackage{xurl}%





\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,fill=black,draw,text=white,inner sep=1.2pt] (char) {#1};}} 			

\newcommand*\builtinlabel[1]{\tikz[baseline=(char.base)]{
	\node[shape=circle,fill=white,draw,text=black,inner sep=0.4pt] (char) {#1};}} 			


\usepackage{etoolbox}
\robustify{\circled}	









\usepackage{xparse}
\newcommand{\BraceSep}{-0.3em}  %

\NewDocumentCommand{\dgal}{sO{}m}{%
  \IfBooleanTF{#1}
    {\dgalext{#3}}%
    {\dgalx[#2]{#3}}%
}

\NewDocumentCommand{\dgalext}{m}{%
  \sbox0{%
    \mathsurround=0pt
    $\left\{\vphantom{#1}\right.\kern-\nulldelimiterspace$%
  }%
  \sbox2{\{}%
  \ifdim\ht0=\ht2
    \{\kern\BraceSep \{#1\}\kern\BraceSep\}%
  \else
    \left\{\kern\BraceSep\left\{#1\right\}\kern\BraceSep\right\}%
  \fi
}

\NewDocumentCommand{\dgalx}{om}{%
  \sbox0{\mathsurround=0pt$#1\{$}%
  \sbox2{\{}%
  \ifdim\ht0=\ht2
    \{\kern\BraceSep \{#2\}\kern\BraceSep\}%
  \else
    \mathopen{#1\{\kern\BraceSep #1\{}%
    #2%
    \mathclose{#1\}\kern\BraceSep #1\}}%
  \fi
}




\makeatletter

\newcommand{\DeclareTarget}[1]{%
  \@bsphack
  \protected@write\@auxout{}{%
    \string\@registertarget{#1}%
  }%
  \@esphack
  \@registertarget{#1}%
}

\newcommand{\@registertarget}[1]{%
  \expandafter\gdef\csname target@#1\endcsname{}%
}

\newcommand{\TargetExists}[1]{%
  \@ifundefined{target@#1}{\@secondoftwo}{\@firstoftwo}%
}

\makeatother

\NewDocumentCommand{\HA}{m o}{%
  \IfNoValueTF{#2}
    {%
      \DeclareTarget{#1}%
      \raisebox{8mm}[0pt][0pt]{\hypertarget{#1}{}}%
      {\color{purple}{#1}}%
    }
    {%
      \DeclareTarget{#2}%
      \raisebox{8mm}[0pt][0pt]{\hypertarget{#2}{}}%
      {\color{purple}{#1}}%
    }%
}

\NewDocumentCommand{\HL}{m o}{%
  \IfNoValueTF{#2}
    {\TargetExists{#1}
      {\hyperlink{#1}{#1}}
      {\textcolor{red}{[Error: Link ``#1'' does not exist]}}}
    {\TargetExists{#2}
      {\hyperlink{#2}{#1}}
      {\textcolor{red}{[Error: Link ``#2'' does not exist]}}}%
}




